Graphical Symplectic Algebra

We give complete presentations for the dagger-compact props of affine Lagrangian and coisotropic relations over an arbitrary field. This provides a unified family of graphical languages for both affinely constrained classical mechanical systems, as well as odd-prime-dimensional stabiliser quantum circuits. To this end, we present affine Lagrangian relations by a particular class of undirected coloured graphs. In order to reason about composite systems, we introduce a powerful scalable notation where the vertices of these graphs are themselves coloured by graphs. In the setting of stabiliser quantum mechanics, this scalable notation gives an extremely concise description of graph states, which can be composed via ``phased spider fusion.'' Likewise, in the classical mechanical setting of electrical circuits, we show that impedance matrices for reciprocal networks are presented in essentially the same way.

==> section_Applications_archive.tex <==
\cole{TODO FLEXSYMMETRIZE}
\cole{TODO ADD ALL CITATIONS  MISSING MANY}

In this section, we review some of the applications of symplectic categories of relations.  We show how the string diagrammatic presentation which is provided in this article provides a unifying equational theory for fragments of quantum mechanical and classically mechanical circuits.  We first will expose the classical side of things, followed by the quantum side.

Symplectic geometry is the geometry of Hamiltonian mechanics.% field is usually chosen to be $\K=\R$.  
The elements of the $Z$ and $X$ gradings of a symplectic vector space are interpreted respectively as abstract {\em positions} and {\em momenta}. In different mechanical settings, there are different notions of positions and momenta:

\begin{figure}
\hfil
\begin{tabular}{||l|llll||}
\hline
 {\it Domain}                        & $Z$        & $\Delta Z$    & $X$                                   & $\Delta X$\\ \hline
{\bf Translation}                    & position & velocity         & momentum                      & force\\
{\bf Electronic}                      & charge   & current          & flux linkage                      & voltage\\
{\bf Hydraulic}                       & volume  & flow               &  pressure momentum      & pressure\\
{\bf Thermal}                         & entropy & entropy flow  & temperature momentum & temperature\\ \hline
\end{tabular}

\caption{
Instantiations of abstract positions $Z$ and momenta $X$.  $\Delta Z$ and $\Delta X$ are the change in position and momentum with respect to time (adapted from \cite{baez???}).
}
\label{fig:mechanics}
\end{figure}

In analogy to how the inner product measures distances,  the symplectic form measures {\em oriented areas}.
The linear symplectomorphisms are the invertible transformations which preserve oriented areas and the origin.
Physically, linear symplectomorphisms capture the Hamiltonian evolution of linear mechanical systems.  We will chose to focus on the example of electrical circuits, although we could just as well pick any row from this table... or even more conceptually, any linear/affine system with an appropriate notion of flow.

The connection between affine Lagrangian relations and electrical circuits is developed in  \cite{passive,network}.  In \cite{passive} they use linear Lagrangian relations to give a semantics for ``passive linear circuits''.  These are an idealized class of electrical circuits with linear behaviour; where the wires have no resistance.
Recall the following physical laws due to Ohm \cite{ohm} followed by Kirchhoff (where we can't find the original reference for the latter):
\begin{description}
\item[Ohm's law:]  The voltage around the node in a circuit is equal to the current multiplied by the resistance.
\item[Kirchhoff's current law:] The sum of currents flowing into a node is equal to the sum of currents flowing out of the node.
\end{description}
This  allows us to capture (linear) resistors as Lagrangian relations.  Given a linear resistor with resistance $r\in \R^{+}$, by Kirchhoff's current  law the incoming current is equal to the outgoing current; and by By Ohm's law, the outgoing potential is equal to the current multiplied by $r$ plus the incoming potential:
$$
\left\llbracket
\begin{circuitikz}
\draw (0,0) to [resistor, R=$r$] (2,0);
\end{circuitikz}
\ \right\rrbracket
=
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=wn,  label={[gphase]below:$0,r$}] (0) at (0, 0) {};
		\node [style=none] (2) at (1, 0) {};
		\node [style=none] (4) at (-1, 0) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (4.center) to (0);
		\draw (0) to (2.center);
	\end{pgfonlayer}
\end{tikzpicture}
$$

Therefore, it is immediate from \ref{spider fusion} that composing resistors in sequence adds resistance.

\cole{DRAW in series}


As opposed to mere symplectomorphisms, Lagrangian relations capture the nondeterministic Hamiltonian evolution of mechanical systems.  In the example of electrical circuits,
this allows us to capture an (ideal) junction with no resistance with $n$ incoming wires and $m$ outgoing wires.  By Kirchhoff's current law, the sum of the currents of the $n$ incoming wires is equal to the sum of the currents of the $m$ outgoing wires.  Moreover, by Ohm's law, because resistance is zero, the $n$ incoming and $m$ outgoing potentials are all made to be equal.  That is to say that the junction is interpreted as the following Lagrangian relation:
$$
\left\llbracket\
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=none] (0) at (3, 0.5) {};
		\node [style=none] (1) at (3, -0.5) {};
		\node [style=none] (2) at (0.5, 0.5) {};
		\node [style=none] (3) at (0.5, -0.5) {};
		\node [style=dot] (4) at (1.75, 0) {};
		\node [style=none] (5) at (2.425, 0.155) {$\vdots$};
		\node [style=none] (6) at (1.075, 0.155) {$\vdots$};
		\node [style=none] (7) at (2.75, 0) {$m$};
		\node [style=none] (8) at (0.75, 0) {$n$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=60, out=180, looseness=0.75] (0.center) to (4);
		\draw [in=0, out=120, looseness=0.75] (4) to (2.center);
		\draw [in=-120, out=0, looseness=0.75] (3.center) to (4);
		\draw [in=180, out=-60, looseness=0.75] (4) to (1.center);
	\end{pgfonlayer}
\end{tikzpicture}
\ \right\rrbracket
=
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=none] (0) at (3, 0.5) {};
		\node [style=none] (1) at (3, -0.5) {};
		\node [style=none] (2) at (0.5, 0.5) {};
		\node [style=none] (3) at (0.5, -0.5) {};
		\node [style=bn] (4) at (1.75, 0) {};
		\node [style=none] (5) at (2.425, 0.155) {$\vdots$};
		\node [style=none] (6) at (1.075, 0.155) {$\vdots$};
		\node [style=none] (7) at (2.75, 0) {$m$};
		\node [style=none] (8) at (0.75, 0) {$n$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=60, out=180, looseness=0.75] (0.center) to (4);
		\draw [in=0, out=120, looseness=0.75] (4) to (2.center);
		\draw [in=-120, out=0, looseness=0.75] (3.center) to (4);
		\draw [in=180, out=-60, looseness=0.75] (4) to (1.center);
	\end{pgfonlayer}
\end{tikzpicture}
$$


Therefore, we find that the general pivoting rule simplifies the behaviour of resistors composed in parallel:

\cole{TODO DRAW COMPOSING RESISTORS IN PARALLEL}

therefore, we see that the reversible Hamiltonian evolution of given by placing two resistors in parallel emerges from the behaviour of all the possible paths which electricity can flow.

This fragment of eletrical circuits has recently been given a complete equational theory \cite{amolakresistors}; their completeness result relies on the ``star-mesh'' transformations, which are linear versions of pivoting.
However, we are working in a larger semantic domain, and therefore more generators can be expressed using our string diagrams.




By working in affine Lagrangian relations, now we can nudge the position of momentum by a constant factor.  For example, recalling \cite{network}, voltage and current sources with voltage $v$ and current $c$ have the following interpretations:

$$
\left\llbracket
\begin{circuitikz}[/tikz/circuitikz/bipoles/length=1cm]
\draw (2,0) to  (0,0);
\node [style=vsourceAMshape, fill=white, xscale=-1] at (1,0) {};
\node [style=none] (3) at (1, 1) {$v$};
\end{circuitikz}
\ \right\rrbracket
=
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=wn,  label={[gphase]below:$v,0$}] (0) at (0, 0) {};
		\node [style=none] (2) at (1, 0) {};
		\node [style=none] (4) at (-1, 0) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (4.center) to (0);
		\draw (0) to (2.center);
	\end{pgfonlayer}
\end{tikzpicture}\ , 
\hspace*{.5cm}
\left\llbracket
\begin{circuitikz}
\draw (2,0) to  (0,0);
\node [style=isourceAMshape, fill=white, xscale=-1] at (1,0) {};
\node [style=none] (3) at (1, 1) {$I$};
\end{circuitikz}
\ \right\rrbracket
=
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=bn, label={[gphase]below:$I,0$}] (0) at (1, 0) {};
		\node [style=none] (1) at (0, 0) {};
		\node [style=bn, label={[gphase]below:$1/I,0$}] (2) at (2.5, 0) {};
		\node [style=none] (3) at (3.5, 0) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (1.center) to (0);
		\draw (3.center) to (2);
	\end{pgfonlayer}
\end{tikzpicture}
$$


This semantics can be augmented further to account for time-dependent components.  The following definition is needed to this end:
\begin{definition}
The {\bf field of real rational functions} is the field of fractions of single variable polynomials over $\R$:

$$
\R(s):= \left\{ \dfrac{f(s)}{g(s)}\  | \ \forall f(s),g(s) \in \R[s], g(s)\neq 0 \right\} 
$$
\end{definition}
In \cite{control}, they interpret ``linear constant-coefficient ordinary differential equations'' relating $n$ inputs to $m$ outputs as $\R(s)$-linear relations from $n$ to $m$.  The multiplication of the polynomial indeterminate $s$ is regarded as differentiation, and multiplication by $s^{-1}$ as integration.   Regarding these differential equations as being dependent on time, in \cite{passive}, they interpret inductors and capacitors as Lagrangian relations over $\R(s)$.  In some sense, the multiplication by the scalar $s$ is interpreted as a discrete step forward in time, and by $s^{-1}$ a discrete step backwards in time. 

A (linear) inductor with inductance $\ell \in \R^+$ is a component with one input and one output such that the voltage is equal to the rate of change of the current multiplied by $\ell$.  Applying Kirchhoff's current law Ohm's law we have that an inductor is interpreted as follows:
$$
\left\llbracket
\begin{circuitikz}
\draw (0,0) to [inductor, L=$\ell$] (2,0);
\end{circuitikz}
\ \right\rrbracket
=
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=gn, label={[rphase]below:$0,-1/(\ell s)$}] (0) at (0, 0) {};
		\node [style=none] (2) at (1, 0) {};
		\node [style=none] (4) at (-1, 0) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (4.center) to (0);
		\draw (0) to (2.center);
	\end{pgfonlayer}
\end{tikzpicture}
$$
Dually, a (linear) capacitor with capacitance $c \in \R^+$ is a component with one input and one output where the current is equal to the rate of change of the voltage multiplied by $c$.  The interpretation is given by:
$$
\left\llbracket
\begin{circuitikz}
\draw (0,0) to [capacitor, C=$c$] (2,0);
\end{circuitikz}
\ \right\rrbracket
=
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=wn,  label={[gphase]below:$0,cs$}] (0) at (0, 0) {};
		\node [style=none] (2) at (1, 0) {};
		\node [style=none] (4) at (-1, 0) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (4.center) to (0);
		\draw (0) to (2.center);
	\end{pgfonlayer}
\end{tikzpicture}
$$

Although, an equational theory for the class of electrical circuits generated by the aforementioned components is still an open question.  To our knowledge, only a partial result exists for networks of resistors \cite{amolakresistors}.
  It is also important to reiterate that the electrical circuits semantics is only one example.  We could have just as easily replaced idealized wires with idealized pipes through which fluid flows, resistors with narrowing pipes and so on.  Or more conceptually, some linear/affine network in which tokens are flowing throughout, where the flow can be assumed to be Hamiltonian.  In any case, we have not just given tools for calculating properties about this networks; the rules are topologically-aware, in the sense that the physical details of equivalent networks respect the topological structure of the implementation of the network.  

This topological nature of circuit diagrams, combined with completeness and universality result which we provide, means that it is no longer necessary to blackbox the behaviour of circuits for these mechanical systems, in the sense of \cite{cite baez' papers}.  Because of the generators-and-relations syntactic presentations we have given are isomorphic to their semantic categories of relations, we have opened up the black box and can now look inside; we have the best of both worlds.


By changing the field from $\R(s)$ to $\mathbb F_p$, for $p$ an odd prime, we capture odd prime dimensional stabilizer circuits (up to scalars).  That is to say, we capture the fragment of quantum circuits which are used extensively in quantum error correction. 

\cole{TODO {\em very} brief overview of quantum circuits and stabilizer formalism for nonexpert.  This would take so much space ugh....}

\cole{TODO give table of all of the interpretations of quantum gates}

 There is a direct comparison between the electrical circuit components and the stabilizer circuit components; however, now there is no total order on the field. For example, the resistors now are precisely the phase-shift gates and the voltage sources are now exactly the Pauli $X$ gates. Note that the ground relation for electrical circuits is an isotropic relation and the quantum discard is a coisotropic relation; despite being drawn using the same symbol, they are orthogonal (they are literally orthogonal complements of each other).

 Stabilizer circuits are the natural setting to do almost all of quantum error correction, and the discard map allows one to implement classical control.


\cole{TODO allude to karoubi envelope and idempotent splitting}


\cole{DRAW BASTARD SPIDER DIAGRAMS BUT DON't define them.  Cite my paper.  Copy paste error correction protocol????}


Because we have given a unified description for these classes of quantum and classical mechanical systems; we have access to all of the tools used for quantum circuit optimization.  For example, the circuit simplyfication tool pyzx \cite{????} already simplifies stabilizer ZX diagrams.  Very minimal changes would be needed in order for this tool to be repurposed for electrical circuits, or indeed, any linear/affine network with Hamiltonian flow.

\cole{Is quopit stabilizer circuits in PYZX?  If we changed a few lines and made it work for real numbers this would look very impressive}

\cole{Robert, can you hint at quantization?  I think the end of this section naturally leads into the conclusion and future work}



